Beyond Black-Box Predictions: Identifying Marginal Feature Effects in Tabular Transformer Networks

In recent years, deep neural networks have showcased their predictive power across a variety of tasks. Beyond natural language processing, the transformer architecture has proven efficient in addressing tabular data problems and challenges the previously dominant gradient-based decision trees in these areas. However, this predictive power comes at the cost of intelligibility: Marginal feature effects are almost completely lost in the black-box nature of deep tabular transformer networks. Alternative architectures that use the additivity constraints of classical statistical regression models can maintain intelligible marginal feature effects, but often fall short in predictive power compared to their more complex counterparts. To bridge the gap between intelligibility and performance, we propose an adaptation of tabular transformer networks designed to identify marginal feature effects. We provide theoretical justifications that marginal feature effects can be accurately identified, and our ablation study demonstrates that the proposed model efficiently detects these effects, even amidst complex feature interactions. To demonstrate the model's predictive capabilities, we compare it to several interpretable as well as black-box models and find that it can match black-box performances while maintaining intelligibility. The source code is available at https://github.com/OpenTabular/NAMpy.

==> old_introduction.tex <==
\section{Version 1: Introduction}


Tabular data analysis has traditionally been dominated by decision tree-based models like XGBoost and Catboost \citep{grinsztajn2022tree, shwartz2022tabular}. Recently, efforts have been made by models that leverage the transformer architecture \citep{vaswani2017attention} such as Tabpfn \citep{hollmann2022tabpfn}, FT-Transformer \citep{gorishniy2021revisiting}, and their predecessors \citep{huang2020tabtransformer, arik2021tabnet} to narrow the performance gap between deep learning models and gradient-boosted decision trees for tabular data. 

Simultaneously, as efforts to enhance model performance continue, there's an increasing push toward making deep learning models more inherently interpretable. The complexity of these high-performing models often categorizes them as "black-boxes," obscuring the reasoning behind their decisions. Typically, explainability for these models is achieved through post-hoc analysis at the sample level, relying on model-agnostic approaches. Techniques like Locally Interpretable Model Explanations (LIME) \citep{ribeiro2016should}, Shapley values \citep{shapley1953quota}, and layer-wise relevance propagation (LRP) \citep{bach2015pixel}, along with their extensions \citep{sundararajan2020many}, aim to explain model predictions through local approximation and feature significance.

To bridge the gap in performance seen with traditional statistical models while preserving interpretability, recent efforts have focused on enhancing visual interpretability by incorporating additivity constraints from Generalized Additive Models (GAMs) \citep{hastie2017generalized} into neural network architectures  \citep{agarwal2021neural, chang2021node, enouen2022sparse}.
Similar to GAMs each feature is fit with a separate shape function. Neural Additive Models (NAMs) \citep{agarwal2021neural} and their extensions have emerged as a powerful yet interpretable solution for tabular data problems.  Depending on the model, shape functions vary from Multi-layer Perceptrons (MLP) \citep{agarwal2021neural, radenovic2022neural, thielmann2023neural} to neural oblivious decision trees \citep{chang2021node}, splines \citep{luber2023structural, rugamer2023semi, rugamer2021deepregression, dubey2022scalable} or ensemble decision trees \citep{nori2019interpretml}.
While these models achieve a degree of interpretability at the feature level through careful regularization \citep{siems2024curve}, they often fall short of the predictive accuracy provided by decision trees or even fully connected Multi-Layer Perceptrons \citep{agarwal2021neural, chang2021node}. Despite various enhancements \citep{dubey2022scalable, radenovic2022neural, enouen2022sparse} improving upon the original NAMs, the trade-off between feature-level interpretability and performance persists. Incorporating higher-order feature interactions has been shown to boost performance \citep{kim2022higher, thielmann2023neural}, but this introduces challenges with identifiability and requires complex networks for each feature interaction. This complexity is compounded in NAMs \citep{agarwal2021neural}, which are inherently complex and struggle with large datasets \citep{anonymous2024interpretable}.

To counteract this, we propose to leverage the flexible tabular deep learning architecture from \cite{gorishniy2021revisiting}. In a nutshell, we use target-aware embeddings \citep{gorishniy2022embeddings} and fit shallow one layer neural networks on uncontextualized embeddings while controlling for all higher order interaction effects and using the uncontextualized embeddings in transformer layers.


Our contributions can be summarized as follows:
\begin{itemize}
    \item[I.] We introduce a fully connected tabular deep learning architecture that enables the identification of marginal feature effects.
    \item[II.] We show that by employing strategic feature dropout, we can achieve identifiability.
    \item[III.] We demonstrate that shallow feature networks are sufficient and can create identifiability with minimal parameter increase, without any loss in performance compared to the FT-Transformer.
\end{itemize}

==> old_stuff/NAMformer_vs_FT.tex <==
\begin{table}[h]
\centering
\caption{Comparison between NAMformer and FT-Transformer with identical hyperparameters on different datasets. 5-fold cross validation was performed. The average performances for both models are not out of the bounds of the standard deviations over the 5-folds. Hence, we find that NAMformer, while producing identifiable marginal effects performs as good as FT-Transformer.}
\begin{tabular}{lcccc}
\toprule
Model & CH & MU & DM & HS \\
\midrule
NAMformer\textsubscript{st} & 0.235 & 0.798 & 0.021 & 0.131\\
& $\pm{\textcolor{gray}{0.013}}$ & $\pm{\textcolor{gray}{0.351}}$& $\pm{\textcolor{gray}{0.001}}$& $\pm{\textcolor{gray}{0.021}}$\\

FT-T\textsubscript{st} & 0.227 & 0.839 & 0.026 & 0.127 \\
& $\pm{\textcolor{gray}{0.011}}$ & $\pm{\textcolor{gray}{0.423}}$& $\pm{\textcolor{gray}{0.002}}$& $\pm{\textcolor{gray}{0.018}}$\\
\hline
NAMformer\textsubscript{oh} & 0.220 & 0.801 & 0.022 & 0.162\\
& $\pm{\textcolor{gray}{0.007}}$ & $\pm{\textcolor{gray}{0.379}}$& $\pm{\textcolor{gray}{0.001}}$& $\pm{\textcolor{gray}{0.021}}$\\

FT-T\textsubscript{oh} & 0.225 & 0.901 & 0.024 & 0.158 \\
& $\pm{\textcolor{gray}{0.007}}$ & $\pm{\textcolor{gray}{0.417}}$& $\pm{\textcolor{gray}{0.002}}$& $\pm{\textcolor{gray}{0.029}}$\\
\hline
NAMformer\textsubscript{ple} & & & & \\
& & & & & \\

FT-T\textsubscript{ple} & & & & \\
& & & & & \\
\bottomrule
\end{tabular}
\label{tab:comparison}
\end{table}

==> old_stuff/ablation_mse_table.tex <==
\begin{table}[h]
\centering
\caption{Average MSE values over marginal feature effects for different datasets. 
With increasing index, the number of effects as well as the complexity of the data increase. Smaller values are better.}
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{7}{c}{Number of marginal effects} \\
\cmidrule(lr){2-8}
Model & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
\midrule
Linear & 0.4583 & 0.5714 & 0.7876 & 1.1825 & 1.5431 & 2.0738 & 2.3553 \\
GAM & 0.1343 & 0.2385 & 0.4659 & 0.6991 & 1.1203 & 1.6426 & 1.9336 \\
EBM & 0.1349 & 0.2392 & 0.4661 & 0.7069 & 1.1234 & 1.6439 & 1.9533 \\
EB\textsuperscript{2}M & 0.1087 & 0.2159 & 0.4363 & 0.6847 & 1.1047 & 1.6201 & 1.9376 \\
NAM & 0.3870 & 0.5032 & 0.7371 & 1.0779 & 1.4468 & 1.9622 & 2.2900 \\
NA\textsuperscript{K}M & 0.0513 & 0.0571 & 0.0634 & 0.0824 & 0.1775 & 0.2116 & 0.2716 \\
NAMformer & 0.0670 & 0.0752 & 0.1860 & 0.1810 & 0.3016 & 0.6747 & 0.9162 \\
\bottomrule
\end{tabular}

\label{tab:mytable}
\end{table}


\begin{table}[htbp]
\centering
\caption{Average R\textsuperscript{2} values over marginal feature effects for different datasets. 
With increasing index, the number of effects as well as the complexity of the data increase. Larger values are better.}
\begin{tabular}{l|ccccccc}

\toprule
& \multicolumn{7}{c}{Number of marginal effects} \\
\cmidrule(lr){2-8}
Model & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
\midrule
Linear & 0.4671 & 0.2513 & 0.2201 & 0.2383 & 0.1236 & 0.0338 & 0.0920 \\
GAM & 0.7989 & 0.5338 & 0.4663 & 0.5004 & 0.3561 & 0.2568 & 0.2992 \\
EBM & 0.7968 & 0.5313 & 0.4640 & 0.4998 & 0.3711 & 0.2656 & 0.3312 \\
EB\textsuperscript{2}M & 0.7968 & 0.5313 & 0.4640 & 0.4998 & 0.3711 & 0.2656 & 0.3312 \\
NAM & 0.7413 & 0.6527 & 0.6106 & 0.6477 & 0.6286 & 0.4771 & 0.5071 \\
Hi-NAM & 0.8009  & 0.5564  & 0.5766 & 0.6762 & 0.5965 & 0.5261  & 0.6580  \\
NAMformer & \textbf{0.8256} & \textbf{0.8774} & \textbf{0.7369} & \textbf{0.8370} & \textbf{0.9223} & \textbf{0.7216} & \textbf{0.8262} \\
\bottomrule
\end{tabular}

\label{tab:ablation_app}
\end{table}

==> old_stuff/old_figures.tex <==
\paragraph{Results}
The results for interpretable models are reported in table \ref{tab:interpretable}. We find that NAMformer performs (shared) best for 6 out of 8 datasets. Additionally, we find strong support for EBMs, with both, EBMs and EB\textsuperscript{2}Ms performing strongly. While NAMs perform only marginally better than classical GAMs and on some datasets even worse, Hi-NAMs also perform strongly, especially on regression tasks. Note, that all models are fine-tuned and hence we achieve different results than for the identically implemented architectures from table \ref{tab:comparison}.



\begin{figure}[htbp]
\centering
% Subfigure 1
\begin{subfigure}[b]{0.42\linewidth} % 45% of the line width
\includegraphics[width=\linewidth]{figures/variable1_NAMformer.png}
\end{subfigure}
\hfill % This will insert a space between the two figures (if needed)
% Subfigure 2
\begin{subfigure}[b]{0.42\linewidth}
\includegraphics[width=\linewidth]{figures/variable2_NAMformer.png}
\end{subfigure}


% Subfigure 3
\begin{subfigure}[b]{0.42\linewidth}
\includegraphics[width=\linewidth]{figures/variable3_NAMformer.png}
\end{subfigure}
\hfill
% Subfigure 4
\begin{subfigure}[b]{0.42\linewidth}
\includegraphics[width=\linewidth]{figures/variable4_NAMformer.png}
\end{subfigure}

\caption{Marginal feature predictions for NAMformer for a simple simulated example with 4 variables and the described data generating process. Over 25 runs, and with only 25 bins, NAMformer accurately identifies the marginal effects.}
\label{fig:four_images}
\end{figure}

==> old_stuff/tables.tex <==
\begin{table}[H]
\centering
\caption{Average R\textsuperscript{2} values over marginal feature effects for different datasets. 
With increasing index, the number of effects as well as the complexity of the data increase. Larger values are better. The gray $\pm$ values denote the standard deviation among the calculated $R^2$ value for the different marginal effects.}
\begin{tabular}{lccccccc}
\toprule
& \multicolumn{7}{c}{Number of marginal effects} \\
\cmidrule(lr){2-8}
Model & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\
\midrule
Linear & 0.467 & 0.251 & 0.220  & 0.238  & 0.124  & 0.034  & 0.092  \\
 & \textcolor{gray}{$\pm0.41$} & \textcolor{gray}{$\pm0.67$} & \textcolor{gray}{$\pm0.62$}  & \textcolor{gray}{$\pm0.59$}  & \textcolor{gray}{$\pm0.63$}  & \textcolor{gray}{$\pm0.68$}  & \textcolor{gray}{$\pm0.68$}  \\
GAM & 0.800 & 0.534 & 0.466 & 0.500 & 0.356 & 0.257 & 0.299 \\
 & \textcolor{gray}{$\pm0.37$} & \textcolor{gray}{$\pm0.76$} & \textcolor{gray}{$\pm0.73$} & \textcolor{gray}{$\pm0.69$} & \textcolor{gray}{$\pm0.76$} & \textcolor{gray}{$\pm0.81$} & \textcolor{gray}{$\pm0.79$} \\
EBM & 0.797 & 0.531 & 0.464 & 0.500 & 0.371 & 0.266 & 0.331 \\
 & \textcolor{gray}{$\pm0.37$} & \textcolor{gray}{$\pm0.76$} & \textcolor{gray}{$\pm0.73$} & \textcolor{gray}{$\pm0.69$} & \textcolor{gray}{$\pm0.73$} & \textcolor{gray}{$\pm0.79$} & \textcolor{gray}{$\pm0.74$} \\
\bottomrule
\end{tabular}
\label{tab:ablation}
\end{table}











\begin{table}[htbp]
    \centering
    \caption{Comparison to interpretable models with default models $\rightarrow$ No hyperparameter tuning performed}
    \begin{tabular}{l|cccccccc}
    \toprule
        Model & CH $\downarrow$ & MU $\downarrow$ &  DM $\downarrow$ & HS $\downarrow$ & AD $\uparrow$ & BA $\uparrow$  & SH $\uparrow$  & FI $\uparrow$  \\
        \hline
        Linear & 0.370 & 0.726 & 0.115 & 0.333 & 0.852 \textcolor{gray}{\footnotesize{82.4\%}} & 0.871 \textcolor{gray}{\footnotesize{88.6\%}}  & 0.764 \textcolor{gray}{\footnotesize{81.5\%}}& 0.754 \textcolor{gray}{\footnotesize{69.3\%}} \\
        GAM & 0.288 & 0.747 & 0.066 & 0.267 & 0.913 \textcolor{gray}{\footnotesize{85.9\%}} & 0.911 \textcolor{gray}{\footnotesize{90.1\%}} & 0.855 \textcolor{gray}{\footnotesize{86.4\%}} & 0.779 \textcolor{gray}{\footnotesize{70.9\%}}\\
        EBM &  0.253 & 0.701 & 0.066 & 0.224 & 0.926 \textcolor{gray}{\footnotesize{87.2\%}} & 0.911 \textcolor{gray}{\footnotesize{89.7\%}} & 0.857 \textcolor{gray}{\footnotesize{85.8\%}} & 0.779 \textcolor{gray}{\footnotesize{70.8\%}}\\
        EB\textsuperscript{2}M & 0.200 & 0.693 & 0.024  & 0.174  & 0.927 \textcolor{gray}{\footnotesize{87.2\%}} & 0.929 \textcolor{gray}{\footnotesize{90.5\%}} & 0.866 \textcolor{gray}{\footnotesize{86.5\%}} & \textbf{0.781} \textcolor{gray}{\footnotesize{70.7\%}}\\
        NAM &  &  &  &  & & & & \\
        NA\textsuperscript{k}M &  &   &  &  & & & & \\
        \hline
        Ours & \textbf{0.189}  & \textbf{0.680}  & \textbf{0.022} & \textbf{0.148}  & 0.927 \textcolor{gray}{\footnotesize{87.2\%}} & 0.931 \textcolor{gray}{\footnotesize{90.8\%}} & \textbf{0.871} \textcolor{gray}{\footnotesize{86.5\%}} & 0.780 \textcolor{gray}{\footnotesize{70.7\%}} \\
        \bottomrule 
    \end{tabular}
    \label{tab:interpretable_app}
\end{table}








\begin{table}[h]
\centering
\caption{Comparison of MSE between NAMformer and FT-Transformer with identical hyperparameters on different datasets. 5-fold cross validation was performed. The average performances for both models are not out of the bounds of the standard deviations over the 5-folds. Hence, we find that NAMformer, while producing identifiable marginal effects performs as good as FT-Transformer.}
\begin{tabular}{lcc}
\toprule
Dataset & NAMformer & FT-Transformer \\
\midrule
Housing & 0.2619 & 0.2655 \\
 & \textcolor{gray}{$\pm0.0134$} & \textcolor{gray}{$\pm0.0111$} \\
Abalone & 0.8440 & 0.8532 \\
 & \textcolor{gray}{$\pm0.0600$} & \textcolor{gray}{$\pm0.0191$} \\
Airbnb & 0.5702 & 0.5540 \\
 & \textcolor{gray}{$\pm0.3649$} & \textcolor{gray}{$\pm0.3363$} \\
CPU small & 0.0468 & 0.0436 \\
 & \textcolor{gray}{$\pm0.0010$} & \textcolor{gray}{$\pm0.0034$} \\
\bottomrule
\end{tabular}
\label{tab:comparison}
\end{table}

% Ich versuch das mal nochmal für andere encodings auch hinzubekommen und auf noch classification datensätze, aber könnte knapp werden mit der Zeit.

==> old_stuff/token_ident.tex <==
\paragraph{From Uncontextual Embeddings to Marginal Predictions}
To understand the potential of \textit{uncontextualized} embeddings as direct representations of raw input features in non-textual data settings, our investigation first examines their role within tabular data models. The proposed NAMformer architecture employs these \textit{uncontextualized} embeddings directly to generate identifiable marginal feature predictions, necessitating a thorough analysis of their capability and effectiveness. By leveraging the \textit{uncontextualized} embeddings, typically used in the initial encoding stages by state-of-the-art language models like those based on the Transformer architecture \citep{vaswani2017attention}, we aim to evaluate their utility without the complex layers of contextualization found in later stages \citep{peters2018dissecting}. This exploration is critical as it may reveal that raw, minimally processed embeddings can sufficiently capture and represent the essential characteristics of the features, potentially simplifying the model architecture while maintaining high predictive accuracy and interpretability.

State-of-the-art language models first create context-insensitive input token representations, known as raw, \textit{uncontextualized} word embeddings. These models subsequently compute $L$ layers of context-dependent representations, culminating in contextualized embeddings of the raw word representations. Our study focuses on the role of these \textit{uncontextualized} embeddings in effectively representing true feature data, providing a focused examination of their effectiveness without the additional contextual processing typical in language models.

\begin{wrapfigure}{r}{0.5\textwidth}
    \includegraphics[width=0.5\textwidth]
    {figures/token_identifiability.png}
    \caption{\small{Average $R^2$ values over all 9 features. The decision trees are fit using either the \textit{uncontextualized} or the contextualized embeddings as training data and the true features as target variables.}}
    \label{fig:enter-label}
\end{wrapfigure}

To generate identifiable feature predictions, we utilize these \textit{uncontextualized} embeddings. In the context of tabular transformer networks, which do not employ positional encodings, the nature of \textit{context} differs significantly from that in transformer models trained on textual data. The \textit{context} added in the transformer layers consists of feature interactions \citep{huang2020tabtransformer}. The \textit{uncontextualized}, raw embeddings, however, are seldom used and are merely a byproduct of the model architecture. Since the input data for numerical features is not tokenized, \textit{token identifiability} \citep{brunner2019identifiability} directly applies to the tabular input data. To confirm that the \textit{uncontextualized} embeddings are not compromised by the subsequent layers during training, we conduct a simple experiment: First, we train a simple tabular transformer model using the California housing dataset\footnote{See appendix for details on the used datasets}. Second, we extract the \textit{uncontextualized} embeddings and analyze how well the true feature data can be recognized. We follow \cite{brunner2019identifiability} and train a set of $J$ simple decision trees $d_t^j: \mathbb{R}^e \rightarrow \mathbb{R}$ on the embedding of every feature $x_j$. The true inputs, $x_j$, serve here as the target variables, whereas the \textit{uncontextualized} embeddings $\mathbb{E}_j(\bm{x}_j)$ are the training features. We investigate how well each feature can be predicted with its contextualized or uncontextualized embedding. We report $R^2$ values and find that \textit{token identifiability} directly transfers to tabular input data and that \textit{uncontextualized} embeddings are nearly perfect representations of the true data, with $R^2$ values of $\geq 0.96$ for different embedding sizes. For further details on the experimental setup, see the appendix.

